Information-theoretic Multimodal Representation Learning for Electrocardiogram Signals

Electrocardiograms (ECGs) are widely used non-invasive measurements of cardiac activity and play a central role in clinical diagnosis. Recent multimodal approaches align ECG signals with clinical reports to incorporate diagnostic semantics, but clinical reports often fail to preserve the rich physiological structure of ECG waveforms, particularly across multiple levels of abstraction ranging from coarse diagnostic categories to fine-grained morphology. To address this limitation, we formulate ECG representation learning from an information-theoretic perspective and derive a tractable objective that jointly preserves signal structure and integrates clinical semantics. Based on this principle, we propose \textbf{MERIT} (Multimodal ECG Representation via Information Theory), a dual-branch pretraining framework combining masked ECG modeling with ECG--text contrastive alignment. Extensive experiments on PTB-XL and additional benchmarks demonstrate consistent improvements over prior methods, including gains exceeding $3%$ F1 on PTB-XL All and $5%$ F1 on SubClass classification. In zero-shot evaluation, MERIT further improves performance by up to $ +2.66\%$ AUC and $ +2.11\%$ F1 on PTB-XL SubClass, while also demonstrating robustness under multiple distribution-shift settings. Moreover, leveraging the learned ECG representations for ECG-conditioned clinical text generation with large language models improves text quality across several metrics, including ROUGE and METEOR. Together, these results demonstrate that MERIT learns more informative and clinically meaningful ECG representations, particularly for fine-grained clinical applications.

==> Method_Phu.tex <==
\section{Method}
We study the problem of learning ECG representations from a paired ECG--text dataset $\mathcal{D} = \{(\textbf{X}_i, \textbf{Y}_i)\}_{i=1}^{N}$, where $\textbf{X}_i \in \mathbb{R}^{C \times T}$ denotes a 12-lead ECG signal with $C=12$ leads and $T$ time steps, and $\textbf{Y}_i$ is the corresponding clinical report represented as a sequence of text tokens. We consider an ECG encoder $g_\theta: \mathbb{R}^{C \times T} \rightarrow \mathbb{R}^{d}$ and a text encoder $h_\phi: \mathcal{Y} \rightarrow \mathbb{R}^{d}$, producing representations $\mathbf{Z} = g_\theta(\mathbf{X})$ and $\mathbf{R} = h_\phi(\mathbf{Y})$ in a shared latent space of dimension $d$.

Our goal is to learn an ECG representation such that
\begin{itemize}
    \item The presentation should capture clinically meaningful concepts by aligning with its paired clinical report. This is achieved by maximizing the mutual information between the ECG and text representations, i.e., $\max_{\theta, \phi} \; \mathrm{I}(\mathbf{Z}; \mathbf{R})$, thereby promoting the encoding of high-level clinical semantics. 
    \item The representation should retain intrinsic physiological structure from the original ECG signal. For 12-lead ECG data, this includes spatio-temporal dependencies, which are essential for characterizing waveform morphology \cite{ecg-soup, STMEM2024}. Following information-maximization principles \cite{hjelm2019learningdeeprepresentationsmutual, lele2025}, this objective is achieved by $\max_{\theta, \phi} \; \mathrm{I}(\mathbf{Z}; \mathbf{X})$, encouraging the representation to preserve fine-grained signal characteristics and their structural relationships. 
\end{itemize}


\begin{figure*}[t]
\centering
\includegraphics[width=0.8\linewidth]{figures/Infomax.pdf}
\label{fig_Infomax}
\caption{
\textbf{Overview of the proposed ECG-text multimodal representation learning framework.} Given a 12-lead ECG signal and corresponding clinical notes, the model learns a shared representation via two complementary objectives. An information maximization (InfoMax) formulation that reconstructs the masked ECG signal using reconstruction loss and aligns ECG and text representations via a cross-modal alignment (CMA) loss.
Together, these objectives promote robust and clinically meaningful multimodal representations.
}
\label{fig:method}
\end{figure*}

\subsection{Multimodal Information Maximization (MMIM)}
Existing multimodal approaches typically emphasize cross-modal alignment, which improves semantic grounding but may suppress signal-specific information. In contrast, signal-only objectives preserve structure but lack semantic meaning. To address this trade-off, we follow the MMIM principle and aim to jointly maximize
\begin{equation}
\max_{\theta,\phi} \; \mathrm{I}(\mathbf{Z}; \mathbf{R}) + \mathrm{I}(\mathbf{Z}; \mathbf{X}),
\label{eq:mmim}
\end{equation}
where $\mathrm{I}(\mathbf{Z}; \mathbf{R})$ captures shared clinical semantics between ECG and text, and $\mathrm{I}(\mathbf{Z}; \mathbf{X})$ encourages preservation of signal-specific physiological information.

Direct optimization of mutual information is intractable. We therefore derive a practical surrogate using standard lower bounds.

\paragraph{Cross-modal alignment (CMA).}
Following \cite{oord2019representationlearningcontrastivepredictive}, the mutual information $\mathrm{I}(\mathbf{Z}; \mathbf{R})$ can be approximated through a symmetric contrastive objective:
\begin{equation}
\mathcal{L}_{\text{CMA}} =
\mathcal{L}_{\mathbf{Z} \rightarrow \mathbf{R}} + \mathcal{L}_{\mathbf{R} \rightarrow \mathbf{Z}},
\label{eq:align}
\end{equation}
where each term is defined using the InfoNCE loss over a batch of size $B$:
\begin{equation}
\mathcal{L}_{\mathbf{Z} \rightarrow \mathbf{R}}
=
-\frac{1}{B}
\sum_{i=1}^{B}
\log
\frac{\exp(s(\mathbf{Z}_i, \mathbf{R}_i)/\tau)}
{\sum_{j=1}^{B}\exp(s(\mathbf{Z}_i, \mathbf{R}_j)/\tau)},
\label{eq:z2r}
\end{equation}
\begin{equation}
\mathcal{L}_{\mathbf{R} \rightarrow \mathbf{Z}}
=
-\frac{1}{B}
\sum_{i=1}^{B}
\log
\frac{\exp(s(\mathbf{Z}_i, \mathbf{R}_i)/\tau)}
{\sum_{j=1}^{B}\exp(s(\mathbf{Z}_j, \mathbf{R}_i)/\tau)}.
\label{eq:r2z}
\end{equation}
Here, $s(\cdot,\cdot)$ denotes a similarity function and $\tau$ is a temperature parameter.

\paragraph{Signal preservation.}
To approximate $\mathrm{I}(\mathbf{Z}; \mathbf{X})$, we follow the variational lower bound of \cite{10.5555/2981345.2981371} and introduce a variational decoder $q_\psi(\mathbf{X}|\mathbf{Z})$:
\begin{equation}
\mathrm{I}(\mathbf{Z}; \mathbf{X})
\geq
\mathbb{E}_{p(\mathbf{X},\mathbf{Z})}
\left[
\log q_\psi(\mathbf{X}|\mathbf{Z})
\right]
+
H(\mathbf{X}).
\label{eq:ba_bound}
\end{equation}
Since $H(\mathbf{X})$ is independent of the model parameters, maximizing this lower bound reduces to maximizing the conditional log-likelihood under $q_\psi(\mathbf{X}|\mathbf{Z})$.

We instantiate the variational decoder with a Gaussian likelihood:
\begin{equation}
q_\psi(\mathbf{X}|\mathbf{Z})
=
\mathcal{N}
\left(
\mathbf{X}; f_\psi(\mathbf{Z}), \sigma^2 \mathrm{I}
\right),
\label{eq:gaussian}
\end{equation}
where $f_\psi(\mathbf{Z})$ is the reconstructed ECG signal and $\sigma^2$ is a fixed variance. Under this assumption, maximizing $\log q_\psi(\mathbf{X}|\mathbf{Z})$ is equivalent to minimizing the reconstruction loss:
\begin{equation}
\mathcal{L}_{\text{rec}}
=
\left\| \mathbf{X} - f_\psi(\mathbf{Z}) \right\|_2^2.
\label{eq:rec}
\end{equation}

\paragraph{Final objective.}
Combining the cross-modal alignment term and the signal preservation term, the final training objective becomes
\begin{equation}
\mathcal{L}
=
\mathcal{L}_{\text{CMA}}
+
\mathcal{L}_{\text{rec}},
\label{eq:final_loss}
\end{equation}
This objective explicitly balances semantic alignment and structural preservation.

\subsection{Multimodal Information Bottleneck (IB)}
\label{sec:IB}
While our formulation is grounded in InfoMax, an alternative perspective is to explicitly focus on the information shared between modalities. The IB principle~\cite{tishby2000informationbottleneckmethod, tishby2015deeplearninginformationbottleneck} provides such a viewpoint by formulating representation learning as:
\begin{equation}
\max \mathrm{I}(\mathbf{Z}; \mathbf{R}) \quad \text{s.t.} \quad \min \mathrm{I}(\mathbf{Z}; \mathbf{X}),
\end{equation}

which encourages retaining only shared information while discarding modality-specific details. In the ECG-text multimodal setting, this objective can be interpreted as improving the alignment between ECG signals and clinical reports while suppressing information unique to the ECG signals. Recent work~\cite{almudévar2025aligningmultimodalrepresentationsinformation} adopts this principle to align multimodal representations in image-text multimodalities.

However, it remains unclear whether this formulation is well-suited for ECG signals. Unlike modalities such as images or text, ECG signals contain rich physiological information (i.e., inter-lead correlations, waveform morphology, and temporal dynamics) that is often not explicitly described in clinical reports. Discarding such information may limit the expressiveness of the learned representations, particularly for tasks that rely on fine-grained signal characteristics.

To answer this question, we draw inspiration from the IB in~\cite{almudévar2025aligningmultimodalrepresentationsinformation} and adapt it to the ECG-text setting by introducing an IB regularization term over paired representations. This allows us to explicitly control the extent to which the learned representation focuses on shared cross-modal information. We combine this term with the cross-modal alignment objective $\mathcal{L}_{\text{CMA}}$, resulting in the following multimodal IB (MIB) objective:
\begin{equation}
\mathcal{L}_{\text{MIB}} = \mathcal{L}_{\text{CMA}} + \lambda_{\text{IB}}\mathcal{L}_{\text{IB}},
\end{equation}
where $\lambda_{\mathrm{IB}}$ controls the strength of the bottleneck regularization. The bottleneck term is defined as:
\begin{equation}
\mathcal{L}_{\text{IB}}
=
\frac{1}{B}
\sum_{i=1}^{B}
\left(1 - \cos(\textbf{Z}_i, \textbf{R}_i)\right)
=
\frac{1}{B}\sum_{i=1}^{B}\left(1 - \hat{\textbf{Z}}_i^{\top}\hat{\textbf{R}}_i\right),
\end{equation}
where $\hat{\textbf{Z}}_i = \textbf{Z}_i / \|\textbf{Z}_i\|_2$ and $\hat{\textbf{R}}_i = \textbf{R}_i / \|\textbf{R}_i\|_2$ denote the $\ell_2$-normalized ECG and text embeddings, respectively.

\subsection{Model Architecture}
The unified objective provides a direct guideline for designing the learning framework. In particular, the two terms correspond to two complementary requirements: preserving information from the ECG signal and aligning representations with clinical semantics. This leads to a dual-branch architecture that explicitly separates structural preservation and semantic alignment.
\paragraph{Masked ECG Modeling.}
We adopt masked ECG modeling to preserve structural information. 
Given an input signal $\mathbf{X}$, a stochastic masking operator produces a partially observed signal $\mathbf{X}^{\text{mask}} = M(\mathbf{X})$, which is encoded by $g_\theta(\cdot)$ to obtain latent representations $\mathbf{Z}^{\text{vis}}$. 
The full latent sequence $\mathbf{Z}^{\text{full}}$ is formed by inserting masked tokens, and a decoder reconstructs the signal as $\hat{\mathbf{X}} = f_\psi(\mathbf{Z}^{\text{full}})$.

Following STMEM~\cite{STMEM2024} with a lightweight TinyViT backbone, this branch captures both local and long-range physiological patterns. 
As shown in Figure~\ref{fig:method}, the reconstructed representations are shared with the semantic branch, enabling joint optimization of structural preservation and semantic alignment.

\paragraph{ECG-text Alignment.}
In parallel, we construct global representations for cross-modal alignment. 
The ECG features $\mathbf{Z}^{\text{vis}}$ are aggregated via average pooling to obtain $\mathbf{Z}$, while the clinical report $\mathbf{Y}$ is encoded by a pretrained MedCPT model $h_\phi(\cdot)$~\cite{Jin_2023} to produce token embeddings, which are similarly pooled to obtain $\mathbf{R}$.

To align two modalities, we map $\mathbf{Z}$ and $\mathbf{R}$ into a shared embedding space using projection heads, yielding $\tilde{\mathbf{Z}}$ and $\tilde{\mathbf{R}}$. 
Cross-modal alignment is enforced via a symmetric contrastive objective $\mathcal{L}_{\text{CMA}}$. As shown in Figure~\ref{fig:method}, this branch aligns paired ECG and text representations while separating mismatched pairs, enabling integration of clinical semantics into the ECG representation.


